Ensembling Neural Networks for Digital Pathology Images Classification and Segmentation

In the last years, neural networks have proven to be a powerful framework for various image analysis problems. However, some application domains have specific limitations. Notably, digital pathology is an example of such fields due to tremendous image sizes and quite limited number of training examples available. In this paper, we adopt state-of-the-art convolutional neural networks (CNN) architectures for digital pathology images analysis. We propose to classify image patches to increase effective sample size and then to apply an ensembling technique to build prediction for the original images. To validate the developed approaches, we conducted experiments with \textit{Breast Cancer Histology Challenge} dataset and obtained 90\% accuracy for the 4-class tissue classification task.

==> content/models.tex <==
\section{Models}
\subsection{Microscopy images classification}

\subsection{Whole-slide images segmentation}
For the segmentation task we introduce a novel architecture, based on U-Net \cite{unet}. It can be regarded as a generalization, which applies additional convolutions to the connections between the downsampling and upsampling branches.

\begin{figure}
  \centering
  \includegraphics[width=0.70\textwidth]{tnet_example}
  \caption{\label{fig:tnet_example}A schematic example of the T-Net architecture.}
\end{figure}

%%% describe what variations of the architecture were used
%%% quality comparison with u-net

